The chemical structure of the Class 0 protostellar envelope NGC 1333 IRAS 4A

It is not well known what drives the chemistry of a protostellar envelope, in particular the role of the stellar mass and the outflows on its chemical enrichment. We study the chemical structure of NGC 1333 IRAS 4A in order to (i) investigate the influence of the outflows on the chemistry, (ii) constrain the age of our object, (iii) compare it with a typical high-mass protostellar envelope. In our analysis we use JCMT line mapping and HIFI pointed spectra. To study the influence of the outflow on the degree of deuteration, we compare JCMT maps of HCO+ and DCO+ with non-LTE (RADEX) models in a region that spatially covers the outflow activity of IRAS 4A. To study the envelope chemistry, we derive empirical molecular abundance profiles for the observed species using the radiative transfer code (RATRAN) and adopting a 1D dust density/temperature profile from the literature. We compare our best-fit observed abundance profiles with the predictions from the time dependent gas grain chemical code (ALCHEMIC). The CO, HCN, HNC and CN abundance require an enhanced UV field which points towards an outflow cavity. The abundances (wrt H2) are 1 to 2 orders of magnitude lower than those observed in the high mass protostellar envelope (AFGL 2591), while they are found to be similar within factors of a few with respect to CO. Differences in UV radiation may be responsible for such chemical differentiation, but temperature differences seem a more plausible explanation. The CH3OH modeled abundance profile points towards an age of > 4x10^4 yrs for IRAS 4A. The spatial distribution of H2D+ differs from that of other deuterated species, indicating an origin from a foreground colder layer (<20 K). The observed abundances can be explained by passive heating towards the high mass protostellar envelope, while the presence of UV cavity channels become more important toward the low mass protostellar envelope.

==> aa.clsV6.0 <==
% This is aa.cls
% A&A DOCUMENT CLASS -- version 6.1 for LaTeX2e
%
% LaTeX document class for Astronomy and Astrophysics journal
%
%%
%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{aa}[2006/06/01 v6.1
^^JLaTeX document class for Astronomy and Astrophysics journal]
\newcommand\@ptsize{}
\newif\if@restonecol
\newif\if@titlepage
\@titlepagefalse
\newif\if@longauth
\@longauthfalse
\newif\if@online
\@onlinefalse
\newif\if@rnote
\@rnotefalse
\newif\if@oldversion
\@oldversionfalse
\newif\if@letter
\@letterfalse

%
\DeclareOption{a4paper}
   {\setlength\paperheight {297mm}% 
    \setlength\paperwidth  {210mm}}
\DeclareOption{letterpaper}
   {\setlength\paperheight {11in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{legalpaper}
   {\setlength\paperheight {14in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{10pt}{\renewcommand\@ptsize{0}}
\DeclareOption{11pt}{\renewcommand\@ptsize{1}}
\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
\DeclareOption{twoside}{\@twosidetrue  \@mparswitchtrue}
\DeclareOption{draft}{\setlength\overfullrule{5pt}}
\DeclareOption{final}{\setlength\overfullrule{0pt}}
\DeclareOption{twocolumn}{\@twocolumntrue}
\DeclareOption{leqno}{\input{leqno.clo}}
\DeclareOption{fleqn}{\input{fleqn.clo}}
\DeclareOption{openbib}{%
  \AtEndOfPackage{%
   \renewcommand\@openbib@code{%
      \advance\leftmargin\bibindent
      \itemindent -\bibindent
      \listparindent \itemindent
      \parsep \z@
      }%
   \renewcommand\newblock{\par}}%
}
%
\DeclareOption{longauth}{\@longauthtrue}
\DeclareOption{rnote}{\@rnotetrue}
\DeclareOption{oldversion}{\@oldversiontrue}
%% January 2008 - abstract
\DeclareOption{traditabstract}{\@oldversiontrue}
\DeclareOption{structabstract}{\@oldversionfalse}
\DeclareOption{letter}{\@lettertrue}
%
\let\if@runhead\iffalse
\DeclareOption{runningheads}{\let\if@runhead\iftrue}
\let\if@envcntreset\iffalse
\DeclareOption{envcountreset}{\let\if@envcntreset\iftrue}
\let\if@envcntsect\iffalse
\DeclareOption{envcountsect}{\let\if@envcntsect\iftrue}
\let\if@referee\iffalse
\DeclareOption{referee}{\let\if@referee\iftrue}
\let\if@onecolumn\iffalse
\DeclareOption{onecolumn}{\let\if@onecolumn\iftrue}
\let\if@nyobjects\iffalse
%
\ExecuteOptions{a4paper,twoside,twocolumn,fleqn,final,10pt,runningheads}
\ProcessOptions
\AtEndOfClass{\mathindent\z@}
%
\if\@ptsize 0
%
   \renewcommand\normalsize{%
      \@setfontsize\normalsize\@xpt{11}%
      \abovedisplayskip 8.55\p@ \@plus4\p@ \@minus5\p@
      \abovedisplayshortskip \z@ \@plus3\p@
      \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
      \belowdisplayskip \abovedisplayskip
      \let\@listi\@listI}
   \normalsize
   \newcommand\small{%
      \@setfontsize\small\@ixpt{10}%
      \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
      \abovedisplayshortskip \z@ \@plus2\p@
      \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
      \def\@listi{\leftmargin\leftmargini
                  \parsep 0\p@ \@plus1\p@ \@minus\p@
                  \topsep 8\p@ \@plus2\p@ \@minus4\p@
                  \itemsep0\p@}%
      \belowdisplayskip \abovedisplayskip
   }
   \newcommand\scriptsize{\@setfontsize\scriptsize\@viipt\@viiipt}
   \newcommand\tiny{\@setfontsize\tiny\@viiipt\@ixpt} 
   \newcommand\large{\@setfontsize\large\@xipt{13}}
   \newcommand\Large{\@setfontsize\Large\@xivpt{16}}
   \newcommand\LARGE{\@setfontsize\LARGE\@xviipt{20}}
   \newcommand\huge{\@setfontsize\huge\@xxpt{24}}
   \newcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}
   %
   \setlength\parindent{15\p@}
   \setlength\smallskipamount{3\p@ \@plus 1\p@ \@minus 1\p@}
   \setlength\medskipamount{6\p@ \@plus 2\p@ \@minus 2\p@}
   \setlength\bigskipamount{12\p@ \@plus 4\p@ \@minus 4\p@}
   \setlength\headheight{12\p@}
   \setlength\headsep   {12\p@} % 
   \setlength\topskip   {10\p@}
   \setlength\footskip{30\p@}
   \setlength\maxdepth{.5\topskip}
   %
   \@settopoint\textwidth
   \setlength\marginparsep {10\p@}
   \setlength\marginparpush{5\p@}
   \setlength\oddsidemargin   {-30\p@}
   \setlength\evensidemargin  {-30\p@}
   \setlength\marginparwidth  {48\p@}
   \setlength\topmargin{-40pt}
   \setlength\footnotesep{8\p@}
   \setlength{\skip\footins}{9\p@ \@plus 4\p@ \@minus 2\p@}
   \setlength\floatsep    {12\p@ \@plus 2\p@ \@minus 2\p@}
   \setlength\textfloatsep{18\p@ \@plus 8\p@ \@minus 6\p@}
   \setlength\intextsep   {18\p@ \@plus 2\p@ \@minus 2\p@}
   \setlength\dblfloatsep    {12\p@ \@plus 2\p@ \@minus 2\p@}
   \setlength\dbltextfloatsep{18\p@ \@plus 8\p@ \@minus 6\p@}
   \setlength\@fptop{0\p@ }
   \setlength\@fpsep{12\p@ }
   \setlength\@fpbot{0\p@ \@plus 1fil}
   \setlength\@dblfptop{0\p@ }
   \setlength\@dblfpsep{12\p@ }
   \setlength\@dblfpbot{0\p@ \@plus 1fil}
   \setlength\partopsep{2\p@ \@plus 1\p@ \@minus 1\p@}
   \def\@listi{\leftmargin\leftmargini
               \parsep \z@
               \topsep 8\p@ \@plus2\p@ \@minus4\p@
               \itemsep\parsep}
   \let\@listI\@listi
   \@listi
   \def\@listii {\leftmargin\leftmarginii
                 \labelwidth\leftmarginii
                 \advance\labelwidth-\labelsep
                 \topsep    \z@
                 \parsep    \topsep
                 \itemsep   \parsep}
   \def\@listiii{\leftmargin\leftmarginiii
                 \labelwidth\leftmarginiii
                 \advance\labelwidth-\labelsep
                 \topsep    \z@
                 \parsep    \topsep
                 \itemsep   \parsep}
   \def\@listiv {\leftmargin\leftmarginiv
                 \labelwidth\leftmarginiv
                 \advance\labelwidth-\labelsep}
   \def\@listv  {\leftmargin\leftmarginv
                 \labelwidth\leftmarginv
                 \advance\labelwidth-\labelsep}
   \def\@listvi {\leftmargin\leftmarginvi
                 \labelwidth\leftmarginvi
                 \advance\labelwidth-\labelsep}
\else
   \input{size1\@ptsize.clo}
\fi
%
\let\footnotesize\small
%
\setlength{\textwidth}{184mm}
\setlength{\textheight}{705pt} 
%
\setlength\lineskip{1\p@}
\setlength\normallineskip{1\p@}
\renewcommand\baselinestretch{}
\setlength\parskip{0\p@ \@plus \p@}
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
%
\setcounter{topnumber}{4}
\renewcommand\topfraction{.9}
\setcounter{bottomnumber}{2}
\renewcommand\bottomfraction{.5}
\setcounter{totalnumber}{6}
\renewcommand\textfraction{.05}
\renewcommand\floatpagefraction{.95}
\setcounter{dbltopnumber}{3}
\renewcommand\dbltopfraction{.9}
\renewcommand\dblfloatpagefraction{.95}
%
\def\ps@headings{%
    \let\@oddfoot\@empty\let\@evenfoot\@empty
    \def\@evenhead{\small\rlap{\thepage}\hfil\leftmark\hfil}%
    \def\@oddhead{\small\hfil\rightmark\hfil\llap{\thepage}}%
    \let\@mkboth\@gobbletwo
    \let\sectionmark\@gobble
    \let\subsectionmark\@gobble
    }
% make indentations changeable
\def\setitemindent#1{\settowidth{\labelwidth}{#1}%
        \leftmargini\labelwidth
        \advance\leftmargini\labelsep
   \def\@listi{\leftmargin\leftmargini
        \labelwidth\leftmargini\advance\labelwidth by -\labelsep
        \parsep=\parskip
        \topsep=\medskipamount
        \itemsep=\parskip \advance\itemsep by -\parsep}}
\def\setitemitemindent#1{\settowidth{\labelwidth}{#1}%
        \leftmarginii\labelwidth
        \advance\leftmarginii\labelsep
\def\@listii{\leftmargin\leftmarginii
        \labelwidth\leftmarginii\advance\labelwidth by -\labelsep
        \parsep=\parskip
        \topsep=\z@
        \itemsep=\parskip \advance\itemsep by -\parsep}}
% labels of description
\def\descriptionlabel#1{\hspace\labelsep #1\hfil}
% adjusted environment "description"
% if an optional parameter (at the first two levels of lists)
% is present, its width is considered to be the widest mark
% throughout the current list.
\def\description{\@ifnextchar[{\@describe}{\list{}{\labelwidth\z@
          \itemindent-\leftmargin \let\makelabel\descriptionlabel}}}
\let\enddescription\endlist
%
\def\describelabel#1{#1\hfil}
\def\@describe[#1]{\relax\ifnum\@listdepth=0
\setitemindent{#1}\else\ifnum\@listdepth=1
\setitemitemindent{#1}\fi\fi
\list{--}{\let\makelabel\describelabel}}
%
\newdimen\logodepth
\logodepth=1.3cm
\newdimen\headerboxheight
\headerboxheight=143pt
\newdimen\betweenumberspace          % dimension for space between
\betweenumberspace=3.33pt            % number and text of titles.
\newdimen\aftertext                  % dimension for space after
\aftertext=5pt                       % text of title.
\newdimen\headlineindent             % dimension for space between
\headlineindent=1.166cm              % number and text of headings.
\def\andname{and}
\def\keywordname{Key words.}
\def\lastandname{, and}
\def\mailname{{\it Correspondence to\/}:}
\def\email#1{{e-mail: \tt#1}}
% Used only by the publisher
\def\AASection#1{}
%
\newcounter{inst}
\newcounter{auth}
\newdimen\instindent
\newbox\authrun
\newtoks\authorrunning
\newbox\titrun
\newtoks\titlerunning

\def\journalname#1{\gdef\@journalname{#1}}
\gdef\@journalname{Astronomy \&\ Astrophysics}

\def\headnote#1{\gdef\@headnote{#1}}
\def\@headnote{}

\def\dedication#1{\gdef\@dedic{#1}}
\def\@dedic{}

\let\@date\undefined

\if@oldversion
\long\def\abstract#1{\gdef\@abstract{#1}}
\else
\long\def\abstract#1#2#3#4#5{\gdef\@abstract{\number@fw@rds=0%
         \if!#1!\advance\number@fw@rds-1 \else{\sffamily\itshape Context.}\ \pickupw@rd#1\\\let\WC@go\relax\fi
         {\sffamily\itshape Aims.}\
         \if!#2! \@latex@error{The second heading "Aims" is mandatory in the abstract}{}
           {\it The second heading "Aims" is mandatory in the abstract}\\
           \else\advance\number@fw@rds+1\pickupw@rd#2\\\let\WC@go\relax\fi
         {\sffamily\itshape Methods.}\
         \if!#3! \@latex@error{The third heading "Methods" is mandatory in the abstract}{}
           {\it The third heading "Methods" is mandatory in the abstract}\\
           \else\advance\number@fw@rds+1\pickupw@rd#3\\\let\WC@go\relax\fi
         {\sffamily\itshape Results.}\
         \if!#4! \@latex@error{The forth heading "Results" is mandatory in the abstract}{}
           {\it The forth heading "Results" is mandatory in the abstract}\\
            \else\advance\number@fw@rds+1\pickupw@rd#4\let\WC@go\relax\fi
         \if!#5! \else\\\advance\number@fw@rds+1{\sffamily\itshape Conclusions.}\ \pickupw@rd#5\let\WC@go\relax\fi
         \ifnum\number@fw@rds>400
         \@latex@error{Around \number\number@fw@rds\space words in the abstract instead of 300}{}
         \else\relax\fi}}
\fi

\def\keywords#1{\gdef\@keywords{#1}}
%% January 2007
\def\topics#1{\gdef\@topics{#1}}
\def\@topics{}


\def\institute#1{\gdef\@institute{#1}}

\def\institutename{\par
 \begingroup
 \parindent=0pt
 \parskip=0pt
 \setcounter{inst}{1}%
 \def\and{\par\stepcounter{inst}%
 \hangindent\instindent
 \noindent
 \hbox to\instindent{\hss$^{\theinst}$\enspace}\ignorespaces}%
 \setbox0=\vbox{\def\thanks##1{}\@institute}
 \ifnum\value{inst}>9\relax\setbox0=\hbox{$^{88}$\enspace}%
                 \else\setbox0=\hbox{$^{8}$\enspace}\fi
 \instindent=\wd0\relax
 \ifnum\value{inst}=1\relax
 \else
   \setcounter{inst}{1}%
   \hangindent\instindent
   \noindent
   \hbox to\instindent{\hss$^{\theinst}$\enspace}\ignorespaces
 \fi
 \small
 \ignorespaces
 \@institute\par
 \endgroup}

\def\offprints#1{\begingroup
\def\protect{\noexpand\protect\noexpand}\xdef\@thanks{\@thanks
\protect\footnotetext[0]{\unskip\hskip-1.5em{\it Send offprint requests
to\/}: \ignorespaces#1}}\endgroup\ignorespaces}

\def\mail#1{\gdef\@mail{#1}}
\def\@mail{}

\def\@thanks{}

\def\@fnsymbol#1{\ifcase#1\or\star\or{\star\star}\or{\star\star\star}%
   \or \dagger\or \ddagger\or
   \mathchar "278\or \mathchar "27B\or \|\or **\or \dagger\dagger
   \or \ddagger\ddagger \else\@ctrerr\fi\relax}

\def\inst#1{\unskip$^{#1}$}
\def\fnmsep{\unskip$^,$}

\def\subtitle#1{\gdef\@subtitle{#1}}
\def\@subtitle{}

\def\msnr#1{\gdef\@msnr{#1}}
\def\@msnr{}

\def\idline#1#2{\gdef\@idline{#1}\setcounter{page}{#2}}
\def\@idline{}
\def\doi#1{\gdef\@doi{DOI: 10.1051/0004-6361:#1}}
\def\@doi{(DOI: will be inserted by hand later)}

\def\headnote#1{\gdef\@headnote{#1}}
\def\@headnote{}

\def\ch@ckobl#1#2{\@ifundefined{@#1}
 {\typeout{A\string&A warning: Missing
\expandafter\string\csname#1\endcsname}%
  \csname #1\endcsname{#2}}
 {}}

\def\ch@ckoblabs#1#2#3#4#5#6{\@ifundefined{@#1}
 {\typeout{A\string&A warning: Missing
\expandafter\string\csname#1\endcsname}%
  \csname #1\endcsname{#2}{#3}{#4}{#5}{#6}}
 {}}

\newif\if@normhead \@normheadtrue
\def\hugehead{\@normheadfalse
\onecolumn
\let\thanks=\footnote
\long\def\@makefntext##1{\parindent\bibindent
     \columnwidth\textwidth\advance\columnwidth -\columnsep
     \divide\columnwidth\tw@\hsize\columnwidth \linewidth\columnwidth
     \noindent\hbox to\parindent{\hss$\m@th^{\@thefnmark}$ }##1}%
}

\newcommand\errorref{\@latex@error{Citations are not allowed in the abstract}{}}
\newenvironment{stopref}{\let\cite\errorref\let\citet\errorref\let\citep\errorref}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This counts the words. This is an extract of  "gvol.sty,
% written by Ivan Andrus (gvol@math.byu.edu)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
  \newcount\number@fw@rds
  \long\def\pickupw@rd#1 {%
    \let\WC@go\pickupw@rd #1
    \advance\number@fw@rds+1
    \expandafter\WC@go
   }
% End of wordcount section

\def\maketitle{\par
\ch@ckobl{journalname}{Noname}
\ch@ckobl{date}{Preprint online version: \today}
\ch@ckobl{title}{A title should be given}
\ch@ckobl{author}{Name(s) and initial(s) of author(s) should be given}
\ch@ckobl{institute}{Address(es) of author(s) should be given}
\if@oldversion
\ch@ckobl{abstract}{An abstract should be given}
\else
\ch@ckoblabs{abstract}{An abstract should be given}{An abstract should be given}
{An abstract should be given}{An abstract should be given}{An abstract should be given}
\fi
\ch@ckobl{keywords}{Keywords should be given}
\begingroup
    \begin{stopref}
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{$^{\@thefnmark}$}%
 \def\lastand{\ifnum\value{inst}=2\relax
                 \unskip{} \andname\
              \else
                 \unskip, \andname\
              \fi}%
 \def\and{\stepcounter{auth}\relax
          \ifnum\value{auth}=\value{inst}%
             \lastand
          \else
             \unskip,
          \fi}%
 \ifnum \col@number=\@ne
   \@maketitle
 \else
   \twocolumn[\@maketitle]%
 \fi
 \thispagestyle{empty}
 \global\@topnum\z@
 \if@normhead
    \@thanks
 \else
    \twocolumn[\vspace{\@tempdima}]
    \addtocounter{page}{-1}
    \if!\the\authorrunning!
       \authorrunning{ }%
    \fi
 \fi
 \if!\@mail!\else
    \footnotetext[0]{\kern-\bibindent\mailname\
    \ignorespaces\@mail}%
 \fi
%
 \if@runhead
    \def\\{\unskip\ \ignorespaces}\def\inst##1{\unskip{}}%
    \def\thanks##1{\unskip{}}\def\fnmsep{\unskip}%
    \def\object##1{##1}%
    \instindent=\textwidth
    \advance\instindent by-2\headlineindent
    \if!\the\titlerunning!\else
      \edef\@title{\the\titlerunning}%
    \fi
    \global\setbox\titrun=\hbox{\small\rm\unboldmath\ignorespaces\@title}%
    \ifdim\wd\titrun>\instindent
       \typeout{^^JA\string&A Warning: Title too long for running head.}%
       \typeout{Please supply a shorter form with \string\titlerunning
                \space prior to \string\maketitle}%
       \global\setbox\titrun=\hbox{\small\rm
       Title Suppressed Due to Excessive Length}%
    \fi
    \xdef\@title{\copy\titrun}%
%
    \if!\the\authorrunning!
    \else
      \setcounter{auth}{1}%
      \edef\@author{\the\authorrunning}%
    \fi
    \ifnum\value{auth}>2
       \def\stripauthor##1\and##2\endauthor{%
       \protected@xdef\@author{##1\unskip\unskip\if!##2!\else
       \ et al.\fi}}%
       \expandafter\stripauthor\@author\and\endauthor
    \else
       \gdef\and{\unskip\ and \ignorespaces}%
       {\def\and{\noexpand\protect\noexpand\and}%
       \protected@xdef\@author{\@author}}
    \fi
    \global\setbox\authrun=\hbox{\small\unboldmath\@author\unskip:
                                 \unhbox\titrun\if@rnote~\itshape\rnotname\fi}%
    \ifdim\wd\authrun>\instindent
    \typeout{^^JA\string&A Warning: The running head built automatically
             from \string\author\space and \string\title
             ^^Jexceeds the pagewidth, please supply a shorter form
             ^^Jwith \string\authorrunning\space and/or
             \string\titlerunning\space prior to \string\maketitle}%
    \global\setbox\authrun=\hbox{\small\rm Please give a shorter version
       with: {\tt\string\authorrunning\space}and/or{\tt\space
       \string\titilerunning\space}prior to{\tt\space\string\maketitle}}%
    \fi
    \xdef\@author{\copy\authrun}%
    \markboth{\@author}{\@author}%
 \fi
%
 \end{stopref}
 \endgroup
 \setcounter{footnote}{0}
 \setcounter{footnote}{0}%
 \global\let\thanks\relax
 \global\let\maketitle\relax
 \global\let\@maketitle\relax
 \global\let\@thanks\@empty
 \global\let\@author\@empty
 \global\let\@date\@empty
 \global\let\@title\@empty
 \global\let\@subtitle\@empty
 \global\let\@abstract\@empty
%%January 2007
 \global\let\@topics\@empty
 \global\let\@keywords\@empty
 \global\let\keywords\relax
 \global\let\title\relax
 \global\let\author\relax
 \global\let\abstract\relax
 \global\let\date\relax
 \global\let\and\relax}

\def\AALogo{\setbox254=\hbox{
\setlength{\tabcolsep}{0pt}
\begin{tabular}{l}
\\[-30pt]
{\fontsize{18}{21}\selectfont\sffamily\bfseries Astronomy} \\[-2.5pt]
{\fontsize{16}{12}\selectfont\sffamily\mdseries \kern8pt\&\raisebox{4pt}{\rule{78pt}{1pt}}} \\[-5pt]
{\fontsize{18}{21}\selectfont\sffamily\bfseries Astrophysics}
\end{tabular}}\copy254}

\def\makeheadbox{{
\hbox to\textwidth{%
\if!\@idline!
\hbox to0pt{\vbox{\hsize=40cc
\baselineskip=12pt\hrule\hbox
{\vrule\kern3pt\vbox{\kern3pt
\hb@xt@ 40cc{{\sl\@journalname}\ manuscript no.~\jobname \hfill\copyright~ESO~\the\year}
\if!\@msnr!\hbox{\today}\else
\hb@xt@ 30cc{\hfil\strut\LARGE\bfseries\smash{\@msnr}}\fi
\kern3pt}\hfil\kern3pt\vrule}\hrule}\hss}\hfill
\else
\vbox{\baselineskip=11pt
\hbox{\@idline}
\hbox{\@doi}
\hbox{\small\rm \copyright~ESO~\the\year}}
\hfill\AALogo
\fi}}}

\def\@maketitle{\newpage
 \normalfont
 \vbox to0pt{\vskip-20pt
 \nointerlineskip
 \makeheadbox\vss}\nointerlineskip
 \if@normhead
    \setbox\authrun=\vbox\bgroup
 \fi
%% January 2007
 \if!\@topics!\vskip32pt\else
 \vskip24pt
 {\fontsize{12}{14}\selectfont\sffamily {\itshape \@topics} \hfill \fontsize{17}{20}\selectfont\sffamily Special feature}
 \vskip12pt
 \fi
 \begin{center}
%% Januray 2007
%% \vskip24pt
 \if@letter{\large \lettername}\fi
 {\LARGE \sffamily\bfseries\boldmath
  \hrule\@height\logodepth\@width\z@
  \pretolerance=10000
  \vspace*{-12pt}
  \pretolerance=10000
 \if!\@headnote!\else
   \noindent
   {\normalfont\itshape\ignorespaces\@headnote\par}\vskip 3.5mm
 \fi
  \noindent\ignorespaces
  \@title
  \if@rnote \\ \itshape \rnotename \fi
  \par}
 \vskip 8pt\relax
 \if!\@subtitle!\else
   {\Large \sffamily\bfseries\boldmath
   \pretolerance=10000
   \noindent\ignorespaces\@subtitle \par}\vskip 10pt
 \fi
%% \lineskip .5em
 \setbox0=\vbox{\setcounter{auth}{1}\def\and{\stepcounter{auth} }%
                \hfuzz=2\textwidth\def\thanks##1{}\@author}%
 \value{inst}=\value{auth}%
 \setcounter{auth}{1}%
 {\large \rmfamily\mdseries \noindent\ignorespaces\@author}
 \if@longauth \else \end{center} \fi
 \vskip6pt
\small\rm
 \if@longauth {\it (Affiliations can be found after the references)}  \else
 \leftskip=.8cm\rightskip=\leftskip
 \institutename\fi
 \vskip 8pt \noindent\@date
 \if!\@dedic!\else
    \par
    \normalsize\it
    \addvspace\baselineskip
    \noindent\@dedic
 \fi
 \if@longauth \end{center} \fi
 \vskip 8pt
 \small\rm
 \if!\@abstract!\else
  \begin{center}
   {\sffamily\bfseries\abstractname}\par
  \end{center}
  \@abstract
 \fi
 \vskip 6pt
 \small\rm
 \if!\@keywords!\else
 \noindent{\sffamily\bfseries\keywordname}\ \@keywords
 \fi
%
 \if@normhead
    \egroup % end of header box
    \@tempdima=\headerboxheight
    \advance\@tempdima by-\ht\authrun
%   \advance\@tempdima by-\pagetotal
    \ifdim\@tempdima>0pt
       \vrule width0pt height\@tempdima
    \fi
    \unvbox\authrun
    \global\@minipagetrue
    \global\everypar{\global\@minipagefalse\global\everypar{}}
 \else
    \typeout{\the\c@auth\space author names and}
    \typeout{\the\c@inst\space institutes processed}
    \global\@tempdima=\pagetotal
    \global\advance\@tempdima by24pt
 \fi
 \vskip24pt
}
%
\DeclareMathAlphabet{\mathsc}{OT1}{cmr}{m}{sc}
\def\testbx{bx}%
\DeclareRobustCommand{\ion}[2]{%
\relax\ifmmode
\ifx\testbx\f@series
{\mathbf{#1\,\mathsc{#2}}}\else
{\mathrm{#1\,\mathsc{#2}}}\fi
\else\textup{#1\,{\mdseries\textsc{#2}}}%
\fi}
%
\def\clearelargs{\def\1{}\def\2{}\def\3{}\def\4{}\count255=0}
\def\druck@lement#1{{}^{\2}_{\3}\mathrm{#1}{}^{\1}_{\4}{}\if@tempswa$\fi}
\DeclareRobustCommand{\element}{\relax\ifmmode\@tempswafalse
\else$\@tempswatrue\fi\clearelargs\def\?{\phantom{0}}\@lement}
\def\@lement#1{\if#1[\expandafter\f@@dargs\else\druck@lement{#1}\fi}
\def\f@@dargs#1]{\advance\count255by\@ne
\expandafter\def\csname\number\count255\endcsname{#1}\@lement}
%
%\def\vec#1{\ensuremath{\mathbf{#1}}}
\def\vec#1{\ensuremath{\mathchoice{\mbox{\boldmath$\displaystyle#1$}}
{\mbox{\boldmath$\textstyle#1$}}
{\mbox{\boldmath$\scriptstyle#1$}}
{\mbox{\boldmath$\scriptscriptstyle#1$}}}}
%
\def\tens#1{\ensuremath{\mathsf{#1}}}
%
\setcounter{secnumdepth}{3}
\newcounter {section}
\newcounter {subsection}[section]
\newcounter {subsubsection}[subsection]
\newcounter {paragraph}[subsubsection]
\newcounter {subparagraph}[paragraph]
\renewcommand\thesection      {\@arabic\c@section}
\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}
\renewcommand\thesubsubsection{\thesubsection .\@arabic\c@subsubsection}
\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}
\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}
%
\def\sectcounterend{.}

\def\@seccntformat#1{\csname the#1\endcsname\sectcounterend
\hskip\betweenumberspace}

\def\@sect#1#2#3#4#5#6[#7]#8{%
  \ifnum #2>\c@secnumdepth
    \let\@svsec\@empty
  \else
    \refstepcounter{#1}%
    \protected@edef\@svsec{\@seccntformat{#1}\relax}%
  \fi
  \@tempskipa #5\relax
  \ifdim \@tempskipa>\z@
    \begingroup
      #6{%
        \@hangfrom{\hskip #3\relax\@svsec}%
          \raggedright
          \hyphenpenalty \@M%
          \interlinepenalty \@M #8\@@par}%
    \endgroup
    \csname #1mark\endcsname{#7}%
    \addcontentsline{toc}{#1}{%
      \ifnum #2>\c@secnumdepth \else
        \protect\numberline{\csname the#1\endcsname}%
      \fi
      #7}%
  \else
    \def\@svsechd{%
      #6{\hskip #3\relax
      \@svsec #8\hskip\aftertext}%
      \csname #1mark\endcsname{#7}%
      \addcontentsline{toc}{#1}{%
        \ifnum #2>\c@secnumdepth \else
          \protect\numberline{\csname the#1\endcsname}%
        \fi
        #7}}%
  \fi
  \@xsect{#5}}

%
% measures and setting of sections
%
\def\section{\@startsection{section}{1}{\z@}%
    {-16dd plus-4pt minus-4pt}{6dd}{\large\sffamily\bfseries}}
\def\subsection{\@startsection{subsection}{2}{\z@}%
    {-16dd}{6dd}{\normalsize\sffamily\itshape}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}%
    {-16dd}{6dd}{\normalsize\sffamily}}
\def\paragraph{\@startsection{paragraph}{4}{\z@}%
    {-16dd}{-1pt}{\normalsize\sffamily}}

\setlength\leftmargini  {\parindent}
\leftmargin  \leftmargini
\setlength\leftmarginii {\parindent}
\setlength\leftmarginiii {1.87em}
\setlength\leftmarginiv  {1.7em}
\setlength\leftmarginv  {.5em}
\setlength\leftmarginvi {.5em}
\setlength  \labelsep  {.5em}
\setlength  \labelwidth{\leftmargini}
\addtolength\labelwidth{-\labelsep}
\@beginparpenalty -\@lowpenalty
\@endparpenalty   -\@lowpenalty
\@itempenalty     -\@lowpenalty
\renewcommand\theenumi{\@arabic\c@enumi}
\renewcommand\theenumii{\@alph\c@enumii}
\renewcommand\theenumiii{\@roman\c@enumiii}
\renewcommand\theenumiv{\@Alph\c@enumiv}
\newcommand\labelenumi{\theenumi.}
\newcommand\labelenumii{(\theenumii)}
\newcommand\labelenumiii{\theenumiii.}
\newcommand\labelenumiv{\theenumiv.}
\renewcommand\p@enumii{\theenumi}
\renewcommand\p@enumiii{\theenumi(\theenumii)}
\renewcommand\p@enumiv{\p@enumiii\theenumiii}
\newcommand\labelitemi{\normalfont\bfseries --}
\newcommand\labelitemii{\normalfont\bfseries --}
\newcommand\labelitemiii{$\m@th\bullet$}
\newcommand\labelitemiv{$\m@th\cdot$}

% redefinition of the "\newtheorem" command.
%
% Usage now:
%
%     \newtheorem{env_nam}{caption}[within]{cap_font}{body_font}
% or  \newtheorem{env_nam}[numbered_like]{caption}{cap_font}{body_font}
% or  \newtheorem*{env_nam}{caption}{cap_font}{body_font}
%
% New is "cap_font" and "body_font". It stands for
% fontdefinition of the caption and the text itself.
%
% "\newtheorem*" gives a theorem without number.
%
% A defined newthoerem environment is used as described
% by Lamport.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\@thmcountersep{}
\def\@thmcounterend{.}

\def\newtheorem{\@ifstar{\@sthm}{\@Sthm}}

% definition of \newtheorem with number

\def\@Sthm#1{\@ifnextchar[{\@othm{#1}}{\@nthm{#1}}}

\def\@xnthm#1#2[#3]#4#5{\expandafter\@ifdefinable\csname #1\endcsname
   {\@definecounter{#1}\@addtoreset{#1}{#3}%
   \expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
     \csname the#3\endcsname \noexpand\@thmcountersep \@thmcounter{#1}}%
   \expandafter\xdef\csname #1name\endcsname{#2}%
   \global\@namedef{#1}{\@thm{#1}{\csname #1name\endcsname}{#4}{#5}}%
                              \global\@namedef{end#1}{\@endtheorem}}}

\def\@ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
   {\@definecounter{#1}%
   \expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
   \expandafter\xdef\csname #1name\endcsname{#2}%
   \global\@namedef{#1}{\@thm{#1}{\csname #1name\endcsname}{#3}{#4}}%
                               \global\@namedef{end#1}{\@endtheorem}}}

\def\@othm#1[#2]#3#4#5{%
  \@ifundefined{c@#2}{\@latexerr{No theorem environment `#2'
  defined}\@eha}%
  {\expandafter\@ifdefinable\csname #1\endcsname
  {\global\@namedef{the#1}{\@nameuse{the#2}}%
  \expandafter\xdef\csname #1name\endcsname{#3}%
  \global\@namedef{#1}{\@thm{#2}{\csname #1name\endcsname}{#4}{#5}}%
  \global\@namedef{end#1}{\@endtheorem}}}}

\def\@thm#1#2#3#4{\refstepcounter
    {#1}\@ifnextchar[{\@ythm{#1}{#2}{#3}{#4}}{\@xthm{#1}{#2}{#3}{#4}}}

\def\@xthm#1#2#3#4{\@begintheorem{#2}{\csname the#1\endcsname}{#3}{#4}%
                    \ignorespaces}

\def\@ythm#1#2#3#4[#5]{\@opargbegintheorem{#2}{\csname
       the#1\endcsname}{#5}{#3}{#4}\ignorespaces}

\def\@begintheorem#1#2#3#4{\trivlist
                 \item[\hskip\labelsep{#3#1\ #2\@thmcounterend}]#4}

\def\@opargbegintheorem#1#2#3#4#5{\trivlist
      \item[\hskip\labelsep{#4#1\ #2\ (#3)\@thmcounterend}]#5}

% definition of \newtheorem* without number

\def\@sthm#1#2{\@Ynthm{#1}{#2}}

\def\@Ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
   {\global\@namedef{#1}{\@Thm{\csname #1name\endcsname}{#3}{#4}}%
    \expandafter\xdef\csname #1name\endcsname{#2}%
    \global\@namedef{end#1}{\@endtheorem}}}

\def\@Thm#1#2#3{\@ifnextchar[{\@Ythm{#1}{#2}{#3}}{\@Xthm{#1}{#2}{#3}}}

\def\@Xthm#1#2#3{\@Begintheorem{#1}{#2}{#3}\ignorespaces}

\def\@Ythm#1#2#3[#4]{\@Opargbegintheorem{#1}
       {#4}{#2}{#3}\ignorespaces}

\def\@Begintheorem#1#2#3{#3\trivlist
                           \item[\hskip\labelsep{#2#1\@thmcounterend}]}

\def\@Opargbegintheorem#1#2#3#4{#4\trivlist
      \item[\hskip\labelsep{#3#1\ (#2)\@thmcounterend}]}

% definition of divers theorem environments

\if@envcntsect
   \def\@thmcountersep{.}
   \newtheorem{theorem}{Theorem}[section]{\bf}{\it}
\else
   \newtheorem{theorem}{Theorem}{\bf}{\it}
   \if@envcntreset
      \@addtoreset{theorem}{section}
   \else
      \@addtoreset{theorem}{chapter}
   \fi
\fi
\newtheorem*{proof}{Proof}{\it}{\rm}
\newtheorem{corollary}[theorem]{Corollary}{\bf}{\it}
\newtheorem{definition}[theorem]{Definition}{\bf}{\rm}
\newtheorem{example}[theorem]{Example}{\it}{\rm}
\newtheorem{exercise}[theorem]{Exercise}{\it}{\rm}
\newtheorem{lemma}[theorem]{Lemma}{\bf}{\it}
\newtheorem{note}[theorem]{Note}{\it}{\rm}
\newtheorem{problem}[theorem]{Problem}{\it}{\rm}
\newtheorem{proposition}[theorem]{Proposition}{\bf}{\it}
\newtheorem{question}[theorem]{Question}{\it}{\rm}
\newtheorem{remark}[theorem]{Remark}{\it}{\rm}
\newtheorem{solution}[theorem]{Solution}{\it}{\rm}

\def\@takefromreset#1#2{%
    \def\@tempa{#1}%
    \let\@tempd\@elt
    \def\@elt##1{%
        \def\@tempb{##1}%
        \ifx\@tempa\@tempb\else
            \@addtoreset{##1}{#2}%
        \fi}%
    \expandafter\expandafter\let\expandafter\@tempc\csname cl@#2\endcsname
    \expandafter\def\csname cl@#2\endcsname{}%
    \@tempc
    \let\@elt\@tempd}

\def\theopargself{\def\@opargbegintheorem##1##2##3##4##5{\trivlist
      \item[\hskip\labelsep{##4##1\ ##2\ ##3}]##5}
                  \def\@Opargbegintheorem##1##2##3##4{##4\trivlist
      \item[\hskip\labelsep{##3##1\ ##2}]}
      }

\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\else\unskip\quad\fi\squareforqed}
%
\newdimen\figgap\figgap=1cc
\long\def\@makesidecaption#1#2{%
   \parbox[b]{\@tempdima}{\captionstyle{\floatlegendstyle
                                         #1\floatcounterend}~#2}}
\def\sidecaption#1\caption{%
\setbox\@tempboxa=\hbox{#1\unskip}%
\if@twocolumn
 \ifdim\hsize<\textwidth\else
   \ifdim\wd\@tempboxa<\columnwidth
      \typeout{Double column float fits into single column -
            ^^Jyou'd better switch the environment. }%
   \fi
 \fi
\fi
\@tempdima=\hsize
\advance\@tempdima by-\figgap
\advance\@tempdima by-\wd\@tempboxa
\ifdim\@tempdima<3cm
    \typeout{\string\sidecaption: No sufficient room for the legend;
             using normal \string\caption. }%
   \unhbox\@tempboxa
   \let\@capcommand=\@caption
\else
   \let\@capcommand=\@sidecaption
   \leavevmode
   \unhbox\@tempboxa
   \hfill
\fi
\refstepcounter\@captype
\@dblarg{\@capcommand\@captype}}

\long\def\@sidecaption#1[#2]#3{\addcontentsline{\csname
  ext@#1\endcsname}{#1}{\protect\numberline{\csname
  the#1\endcsname}{\ignorespaces #2}}\begingroup
    \@parboxrestore
    \@makesidecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}
%
% Online material
\long\def\onlfig#1#2{\AtEndDocument{\Online\setcounter{figure}{#1}\addtocounter{figure}{-1}#2}\setcounter{figure}{#1}}
\long\def\onltab#1#2{\AtEndDocument{\Online\setcounter{table}{#1}\addtocounter{table}{-1}#2}\setcounter{table}{#1}}
\long\def\onllongtab#1#2{\AtEndDocument{\Online\setlength{\LTcapwidth}{\textwidth}\setcounter{table}{#1}%
\addtocounter{table}{-1}\onecolumn#2\twocolumn}\setcounter{table}{#1}}
\long\def\onllongtabL#1#2{\AtEndDocument{\Online\setlength{\LTcapwidth}{\textheight}\setcounter{table}{#1}%
\addtocounter{table}{-1}\onecolumn#2\twocolumn}\setcounter{table}{#1}}
\long\def\longtab#1#2{\setlength{\LTcapwidth}{\textwidth}%
\setcounter{table}{#1}\addtocounter{table}{-1}\onecolumn#2\twocolumn\setcounter{table}{#1}}
\long\def\longtabL#1#2{\setlength{\LTcapwidth}{\textheight}%
\setcounter{table}{#1}\addtocounter{table}{-1}\onecolumn#2\twocolumn\setcounter{table}{#1}}
%
% Define \acknowledgements
\def\acknowledgements{\par\addvspace{6pt}\tiny\rm
\trivlist\item[\hskip\labelsep{\em Acknowledgements.\/}]}
\def\endacknowledgements{\endtrivlist\addvspace{6pt}}
%
\newenvironment{verse}
               {\let\\\@centercr
                \list{}{\itemsep      \z@
                        \itemindent   -1.5em%
                        \listparindent\itemindent
                        \rightmargin  \leftmargin
                        \advance\leftmargin 1.5em}%
                \item\relax}
               {\endlist}
\newenvironment{quotation}
               {\list{}{\listparindent 1.5em%
                        \itemindent    \listparindent
                        \rightmargin   \leftmargin
                        \parsep        \z@ \@plus\p@}%
                \item\relax}
               {\endlist}
\newenvironment{quote}
               {\list{}{\rightmargin\leftmargin}%
                \item\relax}
               {\endlist}
\if@compatibility
\newenvironment{titlepage}
    {%
      \if@twocolumn
        \@restonecoltrue\onecolumn
      \else
        \@restonecolfalse\newpage
      \fi
      \thispagestyle{empty}%
      \setcounter{page}\z@
    }%
    {\if@restonecol\twocolumn \else \newpage \fi
    }
\else
\newenvironment{titlepage}
    {%
      \if@twocolumn
        \@restonecoltrue\onecolumn
      \else
        \@restonecolfalse\newpage
      \fi
      \thispagestyle{empty}%
      \setcounter{page}\@ne
    }%
    {\if@restonecol\twocolumn \else \newpage \fi
     \if@twoside\else
        \setcounter{page}\@ne
     \fi
    }
\fi
% Appendix
\newcounter{append}
\setcounter{append}{0}
\newenvironment{appendix}{\par
\def\@hangfrom##1{\setbox\@tempboxa\hbox{{##1}}%
      \hangindent \parindent\noindent\box\@tempboxa}
\def\@seccntformat##1{\csname theap##1\endcsname\hskip\betweenumberspace}
  \setcounter{section}{\value{append}}%
  \setcounter{subsection}{0}%
  \setcounter{figure}{0}%
  \setcounter{table}{0}%
  \newcommand\theapsection{Appendix \@Alph\c@section:}%
  \newcommand\theapsubsection{\@Alph\c@section.\@arabic\c@subsection.}%
  \newcommand\theapsubsubsection{\theapsubsection\@arabic\c@subsubsection.}%
  \renewcommand\thesection{\@Alph\c@section}%
  \renewcommand\thesubsection{\@Alph\c@section.\@arabic\c@subsection}%
  \renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}%
  \renewcommand\theequation{\@Alph\c@section.\@arabic\c@equation}%
  \renewcommand\thefigure{\@Alph\c@section.\@arabic\c@figure}%
  \renewcommand\thetable{\@Alph\c@section.\@arabic\c@table}%
  \@addtoreset{equation}{section}%
  \@addtoreset{figure}{section}%
  \@addtoreset{table}{section}%
  \def\subfigures{\stepcounter{figure}\setcounter{auth}{\value{figure}}%
  \setcounter{figure}{0}%
  \def\thefigure{\@Alph\c@section\@arabic\c@auth\alph{figure}}%
  \def\resetsubfig{\setcounter{figure}{\value{auth}}}}}
{
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \setcounter{figure}{0}%
  \setcounter{table}{0}%
  \renewcommand\thesection{\c@section}%
  \renewcommand\thesubsection{\@arabic\c@subsection}%
  \renewcommand\thesubsubsection{\@arabic\c@subsubsection}%
  \renewcommand\theequation{\@arabic\c@equation}%
  \renewcommand\thefigure{\@arabic\c@figure}%
  \renewcommand\thetable{\@arabic\c@table}%
  \addtocounter{append}{1}
}
%
\setlength\arraycolsep{2.5\p@}
\setlength\tabcolsep{6\p@}
\setlength\arrayrulewidth{.4\p@}
\setlength\doublerulesep{2\p@}
\setlength\tabbingsep{\labelsep}
\skip\@mpfootins = \skip\footins
\setlength\fboxsep{3\p@}
\setlength\fboxrule{.4\p@}
\renewcommand\theequation{\@arabic\c@equation}
\newcounter{figure}
\renewcommand\thefigure{\@arabic\c@figure}
\def\fps@figure{tbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{\figurename\,\thefigure}
\newenvironment{figure}
               {\@float{figure}}
               {\resetsubfig\end@float}
\newenvironment{figure*}
               {\@dblfloat{figure}}
               {\resetsubfig\end@dblfloat}
\let\resetsubfig\relax
\def\subfigures{\stepcounter{figure}\setcounter{auth}{\value{figure}}%
\setcounter{figure}{0}\def\thefigure{\@arabic\c@auth\alph{figure}}%
\def\resetsubfig{\setcounter{figure}{\value{auth}}}}
\newcounter{table}
\renewcommand\thetable{\@arabic\c@table}
\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{\tablename~\thetable}
\newenvironment{table}
               {\small\@float{table}}
               {\end@float}
\newenvironment{table*}
               {\small\@dblfloat{table}}
               {\end@dblfloat}

\def \@floatboxreset {%
        \reset@font
        \small
        \@setnobreak
        \@setminipage
}

\newlength\abovecaptionskip
\newlength\belowcaptionskip
\setlength\abovecaptionskip{10\p@}
\setlength\belowcaptionskip{0\p@}
\newcommand\leftlegendglue{}

\def\fig@type{figure}

\newdimen\figcapgap\figcapgap=5pt
\newdimen\tabcapgap\tabcapgap=10pt

\@ifundefined{floatlegendstyle}{\def\floatlegendstyle{\bf}}{}
\def\floatcounterend{.}

\long\def\@caption#1[#2]#3{\par\addcontentsline{\csname
  ext@#1\endcsname}{#1}{\protect\numberline{\csname
  the#1\endcsname}{\ignorespaces #2}}\begingroup
    \@parboxrestore
    \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}

\def\capstrut{\vrule\@width\z@\@height\topskip}
\@ifundefined{captionstyle}{\def\captionstyle{\normalfont\small}}{}

\long\def\@makecaption#1#2{%
 \ifx\@captype\fig@type
   \vskip\figcapgap
   \setbox\@tempboxa\hbox{{\floatlegendstyle #1\floatcounterend}
   \capstrut #2}%
   \ifdim \wd\@tempboxa >\hsize
     {\floatlegendstyle #1\floatcounterend} \capstrut #2\par
   \else
     \hbox to\hsize{\leftlegendglue\unhbox\@tempboxa\hfil}%
   \fi
 \else
   {\floatlegendstyle #1\floatcounterend} \capstrut #2\par
   \vskip\tabcapgap
 \fi}
% Define `acknowledgement' environment
\def\acknowledgement{\par\addvspace{17pt}\tiny\rm
\trivlist\item[\hskip\labelsep
{\it\ackname}]}
\def\endacknowledgement{\endtrivlist\addvspace{6pt}}
% Define `noteadd' environment
\def\noteadd{\par\addvspace{17pt}\small\rm
\trivlist\item[\hskip\labelsep
{\it\noteaddname}]}
\def\endnoteadd{\endtrivlist\addvspace{6pt}}

\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\DeclareRobustCommand*\mit{\@fontswitch\relax\mathnormal}
\newcommand\@pnumwidth{1.55em}
\newcommand\@tocrmarg{2.55em}
\newcommand\@dotsep{4.5}
\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
    \section*{\contentsname
        \@mkboth{%
           \MakeUppercase\contentsname}{\MakeUppercase\contentsname}}%
    \@starttoc{toc}%
    }
\newcommand*\l@part[2]{%
  \ifnum \c@tocdepth >-2\relax
    \addpenalty\@secpenalty
    \addvspace{2.25em \@plus\p@}%
    \begingroup
      \setlength\@tempdima{3em}%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      {\leavevmode
       \large \bfseries #1\hfil \hb@xt@\@pnumwidth{\hss #2}}\par
       \nobreak
       \if@compatibility
         \global\@nobreaktrue
         \everypar{\global\@nobreakfalse\everypar{}}%
      \fi
    \endgroup
  \fi}
\newcommand*\l@section[2]{%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.5em}%
    \begingroup
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
      #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
    \endgroup
  \fi}
\newcommand*\l@subsection{\@dottedtocline{2}{1.5em}{2.3em}}
\newcommand*\l@subsubsection{\@dottedtocline{3}{3.8em}{3.2em}}
\newcommand*\l@paragraph{\@dottedtocline{4}{7.0em}{4.1em}}
\newcommand*\l@subparagraph{\@dottedtocline{5}{10em}{5em}}
\newcommand\listoffigures{%
    \section*{\listfigurename
      \@mkboth{\MakeUppercase\listfigurename}%
              {\MakeUppercase\listfigurename}}%
    \@starttoc{lof}%
    }
\newcommand*\l@figure{\@dottedtocline{1}{1.5em}{2.3em}}
\newcommand\listoftables{%
    \section*{\listtablename
      \@mkboth{%
          \MakeUppercase\listtablename}{\MakeUppercase\listtablename}}%
    \@starttoc{lot}%
    }
\let\l@table\l@figure
\newdimen\bibindent
\setlength\bibindent{\parindent}
\def\@biblabel#1{}
\def\@cite#1#2{{#1\if@tempswa , #2\fi}}
\newenvironment{thebibliography}[1]
     {\begingroup\section*{{\normalsize\refname}
        \@mkboth{\refname}{\refname}}\tiny
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
           \leftmargin\bibindent
           \setlength{\itemindent}{-\leftmargin}
           \@openbib@code
           \usecounter{enumiv}%
           \let\p@enumiv\@empty
           \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy\clubpenalty4000\widowpenalty4000%
      \sfcode`\.\@m}
     {\endlist\par\endgroup\if@longauth\kern6pt\hrule\kern6pt\institutename\@longauthfalse\fi
      \def\@noitemerr{\@latex@warning{Empty `thebibliography' environment}}}%


\newcommand\newblock{\hskip .11em\@plus.33em\@minus.07em}
\let\@openbib@code\@empty
\newenvironment{theindex}
               {\if@twocolumn
                  \@restonecolfalse
                \else
                  \@restonecoltrue
                \fi
                \columnseprule \z@
                \columnsep 35\p@
                \twocolumn[\section*{\indexname}]%
                \@mkboth{\MakeUppercase\indexname}%
                        {\MakeUppercase\indexname}%
                \thispagestyle{plain}\parindent\z@
                \parskip\z@ \@plus .3\p@\relax
                \let\item\@idxitem}
               {\if@restonecol\onecolumn\else\clearpage\fi}
\newcommand\@idxitem{\par\hangindent 40\p@}
\newcommand\subitem{\@idxitem \hspace*{20\p@}}
\newcommand\subsubitem{\@idxitem \hspace*{30\p@}}
\newcommand\indexspace{\par \vskip 10\p@ \@plus5\p@ \@minus3\p@\relax}
\renewcommand\footnoterule{%
  \kern-3\p@
  \hrule\@width.4\columnwidth
  \kern2.6\p@}
\newcommand\@makefntext[1]{%
    \noindent
    \hb@xt@\bibindent{\hss\@makefnmark\enspace}#1}
%
\newcommand\listofobjects{\if@nyobjects
  \IfFileExists{\jobname.obj}%
               {\section*{\listobjectname}%
                \@starttoc{obj}}%
               {\begingroup
                   \makeatletter
                   \if@filesw
                      \newwrite\tf@obj
                      \immediate\openout\tf@obj\jobname.obj
                      \relax
                   \fi
                   \global\@nobreakfalse
                \endgroup}\fi
               }
%
\newcommand*\l@obj[2]{\noindent`#1' on page #2\par}
%
\DeclareRobustCommand{\object}[1]{#1\global\let\if@nyobjects\iftrue
\addcontentsline{obj}{obj}{#1}}
%
\newcommand\contentsname{Contents}
\newcommand\listfigurename{List of Figures}
\newcommand\listobjectname{List of Objects}
\newcommand\listtablename{List of Tables}
\newcommand\refname{References}
\newcommand\indexname{Index}
\newcommand\figurename{Fig.}
\newcommand\tablename{Table}
\newcommand\partname{Part}
\newcommand\appendixname{Appendix}
\newcommand\abstractname{ABSTRACT}
\newcommand\rnotename{(Research Note)}
\newcommand\rnotname{(RN)}
\newcommand\lettername{\textsc{Letter to the Editor}}
\newcommand\ackname{Acknowledgements.}
\newcommand\noteaddname{Note added in proof}
\newcommand\today{}
\edef\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}
\setlength\columnsep{12pt}
\setlength\columnseprule{0\p@}
\frenchspacing
\clubpenalty=10000
\widowpenalty=10000
\def\thisbottomragged{\def\@textbottom{\vskip\z@ plus.0001fil
\global\let\@textbottom\relax}}
\pagestyle{headings}
\pagenumbering{arabic}
\if@referee
  \setlength{\textwidth}{0.75\textwidth}
  \def\baselinestretch{1.5}
  \let\AALogo\relax
  \onecolumn
  \AtEndDocument{\listofobjects}
\else
\if@onecolumn
\onecolumn
\else
  \twocolumn
\fi\fi
\sloppy
\flushbottom
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\sq{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\def\sun{\hbox{$\odot$}}
\def\la{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\sim\cr}}}}}
\def\ga{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\sim\cr}}}}}
\def\degr{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\utw{\smash{\rlap{\lower5pt\hbox{$\sim$}}}}
\def\udtw{\smash{\rlap{\lower6pt\hbox{$\approx$}}}}
\def\fd{\hbox{$.\!\!^{\rm d}$}}
\def\fh{\hbox{$.\!\!^{\rm h}$}}
\def\fm{\hbox{$.\!\!^{\rm m}$}}
\def\fs{\hbox{$.\!\!^{\rm s}$}}
\def\fdg{\hbox{$.\!\!^\circ$}}
\def\farcm{\hbox{$.\mkern-4mu^\prime$}}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}
\def\cor{\mathrel{\mathchoice {\hbox{$\widehat=$}}{\hbox{$\widehat=$}}
{\hbox{$\scriptstyle\hat=$}}
{\hbox{$\scriptscriptstyle\hat=$}}}}
\def\sol{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr<\cr}}}}}
\def\sog{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr>\cr}}}}}
\def\lse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\simeq\cr}}}}}
\def\gse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\simeq\cr}}}}}
\def\grole{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.5pt}<\cr}}}}}
\def\leogr{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\noalign{\vskip-1pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip-0.5pt}>\cr}}}}}
\def\loa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\approx\cr}}}}}
\def\goa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\approx\cr}}}}}
\def\diameter{{\ifmmode\mathchoice
{\ooalign{\hfil\hbox{$\displaystyle/$}\hfil\crcr
{\hbox{$\displaystyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\textstyle/$}\hfil\crcr
{\hbox{$\textstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptstyle/$}\hfil\crcr
{\hbox{$\scriptstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptscriptstyle/$}\hfil\crcr
{\hbox{$\scriptscriptstyle\mathchar"20D$}}}}
\else{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}%
\fi}}

\def\getsto{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil
$\displaystyle##$\hfil\cr\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\gets\cr\to\cr}}}}}
\def\lid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr
\noalign{\vskip0.9pt}=\cr}}}}}
\def\gid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr
\noalign{\vskip0.9pt}=\cr}}}}}
\def\bbbr{{\rm I\!R}} %reelle Zahlen
\def\bbbm{{\rm I\!M}}
\def\bbbn{{\rm I\!N}} %natuerliche Zahlen
\def\bbbf{{\rm I\!F}}
\def\bbbh{{\rm I\!H}}
\def\bbbk{{\rm I\!K}}
\def\bbbp{{\rm I\!P}}
\def\bbbone{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}
{\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}
\def\bbbc{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}}}
\def\bbbq{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm
Q$}\hbox{\raise
0.05\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm Q$}\hbox{\raise
0.05\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm Q$}\hbox{\raise
0.05\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.8\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm Q$}\hbox{\raise
0.05\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.8\ht0\hss}\box0}}}}
\def\bbbt{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm
T$}\hbox{\hbox to0pt{\kern0.25\wd0\vrule height0.95\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm T$}\hbox{\hbox
to0pt{\kern0.25\wd0\vrule height0.95\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm T$}\hbox{\hbox
to0pt{\kern0.25\wd0\vrule height0.95\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm T$}\hbox{\hbox
to0pt{\kern0.25\wd0\vrule height0.95\ht0\hss}\box0}}}}
\def\bbbs{{\mathchoice
{\setbox0=\hbox{$\displaystyle\rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.38\wd0\vrule height0.45\ht0\hss}\hbox
to0pt{\kern0.52\wd0\vrule height0.5\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.38\wd0\vrule height0.45\ht0\hss}\hbox
to0pt{\kern0.52\wd0\vrule height0.5\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.38\wd0\vrule height0.45\ht0\hss}\raise0.05\ht0\hbox
to0pt{\kern0.52\wd0\vrule height0.45\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.38\wd0\vrule height0.45\ht0\hss}\raise0.05\ht0\hbox
to0pt{\kern0.52\wd0\vrule height0.45\ht0\hss}\box0}}}}
\def\bbbz{{\mathchoice {\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\scriptstyle Z\kern-0.3em Z$}}
{\hbox{$\sf\scriptscriptstyle Z\kern-0.2em Z$}}}}
\def\ts{\thinspace}
%
% Bibliography and bibfile
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
          % Physical Review C
\def\prd{Phys.~Rev.~D}%
          % Physical Review D
\def\pre{Phys.~Rev.~E}%
          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.~Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
          % Physics Reports
\def\physscr{Phys.~Scr}%
          % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
%
\uchyph=0
% 
\long\def\Online{\if@online\else\@onlinetrue
\clearpage
\def\ps@Onlheadings{%
    \let\@oddfoot\@empty\let\@evenfoot\@empty
    \def\@evenhead{\hfil\leftmark, {\it Online Material p~\thepage}\hfil}%
    \def\@oddhead{\hfil\rightmark, {\it Online Material p~\thepage}\hfil}%
    \let\@mkboth\@gobbletwo
    \let\sectionmark\@gobble
    \let\subsectionmark\@gobble
    }
\setcounter{page}{1}
\pagestyle{Onlheadings}
%% 2008
%% \twocolumn[\vspace*{4cm}\noindent{\sffamily\bfseries\Huge\centerline{Online Material}}]
%% \vfill
%% \clearpage
\fi}
\AtBeginDocument{\@ifpackageloaded{natbib}{\let\bibpreamble\relax\newcommand{\bibfont}{\tiny}%
\renewenvironment{thebibliography}[1]{%
 \bibsection\parindent \z@\bibpreamble\bibfont\list
   {\@biblabel{\arabic{NAT@ctr}}}{\@bibsetup{#1}%
    \setcounter{NAT@ctr}{0}}%
    \ifNAT@openbib
      \renewcommand\newblock{\par}
    \else
      \renewcommand\newblock{\hskip .11em \@plus.33em \@minus.07em}%
    \fi
    \sloppy\clubpenalty4000\widowpenalty4000
    \sfcode`\.=1000\relax
    \let\citeN\cite \let\shortcite\cite
    \let\citeasnoun\cite
 }{\if@longauth\kern6pt\hrule\kern6pt\institutename\@longauthfalse\fi\def\@noitemerr{%
  \PackageWarning{natbib}
     {Empty `thebibliography' environment}}%
  \endlist\vskip-\lastskip}}{}
\@ifpackageloaded{longtable}{%
\def\LT@makecaption#1#2#3{%
  \LT@mcol\LT@cols c{\hbox to\z@{\hss\parbox[t]\LTcapwidth{%
    \small\sbox\@tempboxa{#1{{\bfseries#2.} }#3}%
    \ifdim\wd\@tempboxa>\hsize
      #1{{\bfseries#2.} }#3%
    \else
      \hbox to\hsize{\box\@tempboxa\hfil}%
    \fi
    \endgraf\vskip\baselineskip}%
  \hss}}}}{}
}%AtBeginDocument
%
\endinput
%%
%% End of file `aa.cls'.

